Probabilistic Sensor Fusion for Ambient Assisted Living

There is a widely-accepted need to revise current forms of health-care provision, with particular interest in sensing systems in the home. Given a multiple-modality sensor platform with heterogeneous network connectivity, as is under development in the Sensor Platform for HEalthcare in Residential Environment (SPHERE) Interdisciplinary Research Collaboration (IRC), we face specific challenges relating to the fusion of the heterogeneous sensor modalities. We introduce Bayesian models for sensor fusion, which aims to address the challenges of fusion of heterogeneous sensor modalities. Using this approach we are able to identify the modalities that have most utility for each particular activity, and simultaneously identify which features within that activity are most relevant for a given activity. We further show how the two separate tasks of location prediction and activity recognition can be fused into a single model, which allows for simultaneous learning an prediction for both tasks. We analyse the performance of this model on data collected in the SPHERE house, and show its utility. We also compare against some benchmark models which do not have the full structure,and show how the proposed model compares favourably to these methods

==> acronyms.tex <==

\acrodef{EPSRC}{Engineering and Physical Sciences Research Council}
\acrodef{SPHERE}{Sensor Platform for HEalthcare in Residential Environment}
\acrodef{IRC}{Inter\-disciplinary Research Collaboration}
\acrodef{CRF}{Conditional Random Field}
\acrodef{L-CRF}{Linear Chain \ac{CRF}}
\acrodef{IID}[iid]{Independent and Identically Distributed}
\acrodef{NLP}{Natural Language Processing}
\acrodef{SVM}{Support Vector Machine}
\acrodef{RBF}{Radial Basis Function}
\acrodef{RF}{Random Forest}
\acrodef{LR}{Logistic Regression}
\acrodef{POS}{Part of Speech}
\acrodef{LR}{Logistic Regression}
\acrodef{ODC}{Occasionally Dishonest Casino}
\acrodef{CASAS}{Centre for Advanced Studies in Adaptive Systems}
\acrodef{PIR}{Passive Infra-Red}
\acrodef{ADL}{Activities of Daily Living}
\acrodefplural{ADL}{Activities of Daily Living}
\acrodef{AAL}{Ambient Assisted Living}
\acrodef{MLE}{Maximum Likelihood Estimate}
\acrodef{RBF}{Radial Basis Function}
\acrodef{RKHS}{reproducing kernel Hilbert space}
\acrodef{HMM}{Hidden Markov Model}
\acrodef{AR}{Activity Recognition}
\acrodef{ERM}{Empirical Risk Minimisation}
\acrodef{AC}{Auto-correlation}
\acrodef{GP}{Gaussian Process}
\acrodef{EP}{Expectation Propagation}
\acrodef{BPM}{Bayes Point Machine}
\acrodef{MKL}{Multiple Kernel Learning}
\acrodef{MVL}{Multi-View Learning}
\acrodef{MSL}{Multi-Source Learning}
\acrodef{VMP}{Variational Message Passing}
\acrodef{EP}{Expectation Propagation}
\acrodef{RSSI}{Received Signal Strength Indication}
\acrodef{NTP}{network time protocol}
\acrodef{QoS}{Quality of Service}
\acrodef{RGB}{Red-Green-Blue}
\acrodef{RGBD}{RGB-Depth}
\acrodef{BP}{Belief Propagation}


==> sections/04_related_sphere.tex <==
\section{Related Work 2: SPHERE}
\label{sec:related_sphere}

\todoNT{Related work for SPHERE challenge \ie the approaches taken by the participants}

\todoALL{Better name and/or place for this section?}





==> sections/07_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\todoMK{More on artificial data?}

\todoALL{Obviously experiments on the SPHERE challenge dataset, but are there other datasets that we could also use?}

\todoALL{Tables of results etc}

\todoALL{Some nice visualisations to demonstrate fusion}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


